The $O(\alpha^2)$ Initial State QED Corrections to $e^+e^- \rightarrow \gamma^*/Z_0^*$

We calculate the complete $O(\alpha^2)$ initial state radiation corrections to $e^+ e^-$ annihilation into a neutral vector boson in a direct analytic computation without any approximation. The corrections are represented in terms of iterated incomplete (elliptic) integrals over alphabets of square--root valued letters. Performing the limit $s \gg m_e^2$, we find discrepancies with the earlier results of Ref.~\cite{Berends:1987ab} and confirm results obtained in Ref.~\cite{Blumlein:2011mi} where the effective method of massive operator matrix elements has been used, which works for all but the power corrections in $m^2_e/s$. In this way, we also confirm the validity of the factorization of massive partons in the Drell--Yan process. We add non--logarithmic terms at $O(\alpha^2)$ which have not been considered in previous calculations. The final results in the limit $s \gg m_e^2$ can be given in terms of Nielsen integrals.

==> hh.tex <==
\begin{eqnarray}
   HHlat &=& 16 \Biggl\{ - 2 \frac{1+z^2}{1-z} (L-1)^2 \ln(\ep)
    + \Biggl\{\frac{1+z^2}{1-z} \left[2 \ln(1-z) -\frac{1}{2} \ln(z)\right] - 1+z +\frac{1}{2}(1+z) 
    \nonumber\\ &&
    \times \ln(z) \Biggr\} L^2
    +\Biggl\{ \frac{1+z^2}{1-z}[-4\ln(1-z) +\ln(z)] - z\ln(z) +\frac{7}{2}(1-z) + \frac{1}{4}(1+z) 
    \nonumber\\ &&
    \times \ln^2(z) \Biggr\} L
    - \frac{1+z^2}{1-z} \Biggl[S_{1,2}(1-z) + \frac{1}{2} \ln(z) \Li_2(1-z) + \frac{3}{2} \ln^2(z) - \left(\frac{7}{6} + 
    \zeta_2\right) 
    \nonumber\\ &&
    \times \ln(z) 
    - 2 \ln(1-z) \Biggr] 
    - \frac{1}{2}(1+z) (\Li_3(1-z) + 2 S_{1,2}(1-z)) 
    -\frac{2}{3} z\zeta_2 
    \nonumber\\ &&
    - \frac{1}{6} (3+4z) \Li_2(1-z) 
    - \frac{1}{6} (10 - 25 z) \ln(z)  
    + \frac{2}{(1-z)^2} \ln^2(z) - \frac{1}{12}(3 + 28 z) \ln^2(z) 
    \nonumber\\ &&
    + \frac{1}{2}(1-z) - \frac{2}{3} \frac{z}{1-z} \Biggl[1 + \frac{2}{1-z} \ln(z) 
    + \frac{1}{(1-z)^2} \ln^2(z) \Biggr] \Biggr\} \nonumber\\
\end{eqnarray}
